Large Spectral Density Matrix Estimation by Thresholding

Spectral density matrix estimation of multivariate time series is a classical problem in time series and signal processing. In modern neuroscience, spectral density based metrics are commonly used for analyzing functional connectivity among brain regions. In this paper, we develop a non-asymptotic theory for regularized estimation of high-dimensional spectral density matrices of Gaussian and linear processes using thresholded versions of averaged periodograms. Our theoretical analysis ensures that consistent estimation of spectral density matrix of a $p$-dimensional time series using $n$ samples is possible under high-dimensional regime $\log p / n \rightarrow 0$ as long as the true spectral density is approximately sparse. A key technical component of our analysis is a new concentration inequality of average periodogram around its expectation, which is of independent interest. Our estimation consistency results complement existing results for shrinkage based estimators of multivariate spectral density, which require no assumption on sparsity but only ensure consistent estimation in a regime $p^2/n \rightarrow 0$. In addition, our proposed thresholding based estimators perform consistent and automatic edge selection when learning coherence networks among the components of a multivariate time series. We demonstrate the advantage of our estimators using simulation studies and a real data application on functional connectivity analysis with fMRI data.

==> graveyard.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    OLD SAMPLE SPLITTING ALGORITHM    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse
\begin{algorithm}
\caption{Sample splitting} \label{al1}
\begin{tabbing}
   \enspace Initial two sets $\{J\}_{1, \nu} = 0$, $\{J\}_{2, \nu} = \{-m, \cdots,  m\}\setminus \{0\}$\\
   \enspace Randomly select pairs of symmetric elements from $\{J\}_{2, \nu}$, e.g. $\{-1, 1\}$ and put them into \\\
   $\{J\}_{1, \nu}$ until the sizes of the two sets are balanced\\
   \enspace At the end, $\{J\}_{2, \nu} \leftarrow \{J\}_{2, \nu}\cup \{0\}$
\enspace 
\end{tabbing}
\end{algorithm}

\begin{algorithm}
\caption{Tuning threshold value} \label{al2}
\begin{tabbing}
   \enspace Calculate periodograms $I(\omega_j)$ for multiple time series data, where $j \in \{1, \cdots, [n/2]\}$\\
   \enspace For $j \in \{1, \cdots, [n/2]\}$ \\
   \qquad Split the periodograms in the smoothing span from $j-m, \cdots, j+m$, which is used for the \\\
   estimation of $f(\omega_j)$, into two pieces for $N$ times according to Algorithm \ref{al1}.\\
   \qquad For $\nu = 1$ to $\nu = N$ \\\
   \qquad\qquad Calculate $S_{\lambda}(\hat{f}_{1,\nu}(\omega_j))$, $\hat{f}_{2,\nu}(\omega_j)$, $\hat{R}(\omega_j,\lambda)$ for each $\lambda_j$ in a set of grids \\
   \qquad Find $\hat{\lambda}_j$ which minimize $\hat{R}(\omega_j,\lambda)$
\enspace 
\end{tabbing}
\end{algorithm}


Let $\hat{f}_{1,\nu}(\omega_j), ~ \hat{f}_{2,\nu}(\omega_j)$ be the empirical spectral densities based on the $m_1$ and $m_2$ periodograms split above. Let $\hat{\lambda}_j = \argmin \hat{R}(\omega_j,\lambda)$, where
\begin{align*}
\hat{R}(\omega_j,\lambda) := \frac 1 N \sum_{\nu = 1}^N \|T_{\lambda}(\hat{f}_{1,\nu}(\omega_j)) - \hat{f}_{2,\nu}(\omega_j)\|_F^2.
\end{align*}


Then for each frequency $j \in \{1, \cdots, [n/2]\}$, we follow Algorithm \ref{al2} to get an estimate of $\lambda$.

----------------------------------
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SIMULATION: PERFORMANCE METRICS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse

{\color{red} 
---------------------

[Yiming]: Current F1 measures are low, especially for VAR setting. Can we try the following global (across freqs) measures of precision/recall and see if the results improve?

\begin{eqnarray}
    && \text{precision} = % n^{-1}\sum_{j  \in F_n} 
    \frac{\# \{(r,s): ~ r \neq s,  |\hat{f}_{rs}(\omega_j)|\neq 0 \mbox{ for some $\omega_j$}, ~ |f_{rs}(\omega_j)|\neq 0  \mbox{ for some $\omega_j$}\}}{\# \{(r,s): ~ |\hat{f}_{rs}(\omega_j)|\neq 0 \mbox{ for some $\omega_j$} \}} \nonumber \\
    && \text{recall} = \frac{\# \{(r,s): ~ r \neq s, |\hat{f}_{rs}(\omega_j)|\neq 0 \mbox{ for some $\omega_j$} , ~ |f_{rs}(\omega_j)|\neq 0 \mbox{ for some $\omega_j$} \}}{\# \{(r,s): ~ |f_{rs}(\omega_j)|\neq 0 \mbox{ for some $\omega_j$} \}} \nonumber \\
    && \text{F1} =  2\times (\text{precision} \cdot \text{recall})/(\text{precision} + \text{recall}). \nonumber 
\end{eqnarray}

In other words, we define the true graph of marginal dependence among the $p$ time series as  $G := \{ (r,s):  r \neq s, f_{rs}(\omega_j) \neq 0 \mbox{ for some $\omega_j$} \}$ and the estimated graph $\hat{G}$ accordingly. Then we report precision, recall and F1 measures of the estimated graph $\hat{G}$.

-------------------------

}
\fi


==> rmise_he_table.tex <==
\tiny
\begin{table}[p]
\def~{\hphantom{0}}
\tbl{RMISE (in $10^{-2}$) Under Heterogeneous Setting}{%
\begin{tabular}{l@{\hskip 0.4in}ccccc}
%\\
\\
& Smoothed   & Shrinkage& Hard Threshold   & Lasso & Adaptive Lasso\\
\\VMA & & & & &\\
p = 12 & & & & &\\
\multicolumn{1}{r}{n = 200}&35.42(2.39)&10.89(0.6)&10.35(1.3)&9.6(1.24)&9.9(1.24)\\
\multicolumn{1}{r}{n = 400}&24.87(1.54)&9.34(0.22)&8.46(0.46)&8.13(0.51)&8.33(0.5)\\
p = 24 & & & & &\\
\multicolumn{1}{r}{n = 200}&65.34(3.44)&12.71(0.61)&11.92(0.49)&11.36(0.55)&11.59(0.58)\\
\multicolumn{1}{r}{n = 400}&52.31(2.07)&11.69(0.44)&9.67(0.38)&8.72(0.44)&9.13(0.42)\\
p = 48 & & & & &\\
\multicolumn{1}{r}{n = 200}&138.35(6.32)&14.14(0.56)&12.54(0.44)&11.84(0.32)&12.15(0.35)\\
\multicolumn{1}{r}{n = 400}&101.28(3.52)&13.03(0.51)&11.15(0.49)&10.23(0.46)&10.58(0.49)\\
VAR & & & & &\\
p = 12 & & & & &\\
\multicolumn{1}{r}{n = 200}&33.28(2.91)&15.81(1.1)&15.08(1.5)&13.11(1.42)&14.15(1.32)\\
\multicolumn{1}{r}{n = 400}&24.46(2.6)&13.46(0.69)&12.44(1.4)&11.36(0.69)&12.1(0.76)\\
p = 24 & & & & &\\
\multicolumn{1}{r}{n = 200}&60.83(4.55)&20.79(0.72)&19.32(0.41)&17.47(0.3)&18.15(0.35)\\
\multicolumn{1}{r}{n = 400}&45.1(3.03)&18.31(0.86)&16.33(0.53)&14.38(0.41)&15.3(0.41)\\
p = 48 & & & & &\\
\multicolumn{1}{r}{n = 200}&117.25(4.27)&24.68(0.75)&21.43(0.68)&20.08(0.93)&20.78(0.87)\\
\multicolumn{1}{r}{n = 400}&87.93(2.08)&22.07(0.27)&18.83(0.32)&16.54(0.3)&17.38(0.29)\\
\end{tabular}}
\label{table:rmise-heterogeneous}
\begin{tabnote}
\end{tabnote}
\end{table}

==> rmise_ho_heavy_tail_table.tex <==
\begin{table}[p]
\def~{\hphantom{0}}
\tbl{RMISE (in $10^{-2}$) Under Homogeneous Setting}{%
\begin{tabular}{l@{\hskip 0.4in}ccccc}
%\\
\\
& Smoothed   & Shrinkage& Hard Threshold  & Lasso & Adaptive Lasso\\
\\
VMA & & & & &\\
p = 12 & & & & &\\
\multicolumn{1}{r}{n = 100}&43.0(6.9)&21.86(1.55)&27.79(2.38)&23.03(2.06)&25.71(1.97)\\
\multicolumn{1}{r}{n = 200}&30.01(2.92)&17.94(1.06)&20.79(1.72)&16.5(1.7)&18.78(1.72)\\
p = 24 & & & & &\\
\multicolumn{1}{r}{n = 100}&83.54(9.28)&26.43(1.69)&29.97(1.34)&26.25(1.31)&28.3(1.18)\\
\multicolumn{1}{r}{n = 200}&60.66(4.13)&23.01(0.87)&25.98(1.07)&19.5(1.28)&22.47(1.3)\\
p = 48 & & & & &\\
\multicolumn{1}{r}{n = 100}&166.63(10.24)&29.97(1.25)&30.55(0.64)&28.65(0.82)&29.82(0.65)\\
\multicolumn{1}{r}{n = 200}&117.72(4.42)&26.82(0.62)&28.22(0.35)&22.72(0.77)&25.43(0.69)\\
p = 96 & & & & &\\
\multicolumn{1}{r}{n = 100}&327.02(12.36)&32.5(1.24)&30.44(0.52)&29.78(0.44)&30.24(0.46)\\
\multicolumn{1}{r}{n = 200}&235.36(6.87)&29.58(0.71)&28.84(0.29)&25.48(0.5)&27.45(0.42)\\
VAR & & & & &\\
p = 12 & & & & &\\
\multicolumn{1}{r}{n = 100}&38.11(11.37)&37.03(5.11)&40.73(8.13)&39.66(6.79)&42.08(6.62)\\
\multicolumn{1}{r}{n = 200}&32.82(7.72)&25.55(6.1)&33.1(9.0)&29.82(7.14)&34.4(5.71)\\
p = 24 & & & & &\\
\multicolumn{1}{r}{n = 100}&70.46(16.71)&49.26(4.42)&49.32(5.16)&44.78(3.91)&47.37(4.47)\\
\multicolumn{1}{r}{n = 200}&51.62(2.11)&36.49(0.41)&39.19(0.09)&33.43(2.35)&37.07(1.91)\\
p = 48 & & & & &\\
\multicolumn{1}{r}{n = 100}&135.03(23.74)&62.23(5.89)&49.81(4.15)&47.4(2.26)&48.45(2.19)\\
\multicolumn{1}{r}{n = 200}&106.2(2.49)&50.44(1.29)&45.22(1.54)&39.87(1.17)&43.55(2.05)\\
p = 96 & & & & &\\
\multicolumn{1}{r}{n = 100}&265.16(37.98)&76.0(5.87)&49.4(1.97)&48.45(1.45)&48.7(1.51)\\
\multicolumn{1}{r}{n = 200}&217.08(7.34)&60.11(1.3)&45.09(1.1)&43.39(0.92)&44.54(0.86)\\
\end{tabular}}
\label{table:rmise-homogeneous}
\begin{tabnote}
\end{tabnote}
\end{table}

==> rmise_ho_table.tex <==
\begin{table}[p]
\def~{\hphantom{0}}
\tbl{RMISE (in $10^{-2}$) Under Homogeneous Setting}{%
\begin{tabular}{l@{\hskip 0.4in}ccccc}
%\\
\\
& Smoothed   & Shrinkage& Hard Threshold  & Lasso & Adaptive Lasso\\
\\
VMA & & & & &\\
p = 12 & & & & &\\
\multicolumn{1}{r}{n = 200}&29.9(1.41)&17.07(0.6)&23.23(1.14)&17.65(1.15)&20.6(0.95)\\
p = 24 & & & & &\\
\multicolumn{1}{r}{n = 200}&55.74(2.64)&22.13(0.44)&26.79(0.16)&21.01(0.62)&24.1(0.44)\\
p = 48 & & & & &\\
\multicolumn{1}{r}{n = 200}&115.58(5.43)&25.01(0.53)&28.3(0.46)&23.69(0.4)&26.14(0.32)\\
VAR & & & & &\\
p = 12 & & & & &\\
\multicolumn{1}{r}{n = 200}&20.88(1.71)&18.65(1.94)&25.89(3.26)&21.1(2.99)&23.43(3.25)\\
p = 24 & & & & &\\
\multicolumn{1}{r}{n = 200}&39.47(1.52)&27.09(0.49)&33.49(1.63)&25.75(0.88)&28.8(1.41)\\
p = 48 & & & & &\\
\multicolumn{1}{r}{n = 200}&83.22(2.74)&35.63(0.53)&40.07(0.66)&30.07(1.1)&33.3(0.89)\\
\end{tabular}}
\label{table:rmise-homogeneous}
\begin{tabnote}
\end{tabnote}
\end{table}

==> three_metric_he_table.tex <==
\tiny
\begin{table}[p]
\def~{\hphantom{0}}
\tbl{Precision, Recall, F1 Score Under Heterogeneous Setting 1}{%
\begin{tabular}{l@{\hskip 0.4in} ccc ccc ccc}
& \multicolumn{3}{c}{Hard Thresholding}  & \multicolumn{3}{c}{Lasso} & \multicolumn{3}{c}{Adaptive Lasso}\\
VMA & precision & recall & F1 & precision & recall & F1 & precision & recall & F1\\
 p = 12 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&36.1(6.08)&73.33(7.3)&55.53(5.68)&22.72(1.04)&96.0(3.27)&36.71(1.18)&36.1(6.08)&82.67(5.33)&50.11(6.7)\\
\multicolumn{1}{r}{n = 400}&27.47(3.44)&76.0(3.27)&56.32(13.02)&21.85(0.9)&98.67(2.67)&35.77(1.3)&27.47(3.44)&89.33(8.0)&41.94(4.61)\\
 p = 24 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&55.72(14.13)&55.76(1.48)&65.53(1.67)&29.02(3.25)&73.94(8.04)&41.44(3.29)&55.72(14.13)&59.39(2.42)&56.53(7.01)\\
\multicolumn{1}{r}{n = 400}&34.24(8.91)&58.18(1.21)&61.16(4.9)&15.73(2.33)&85.45(7.52)&26.39(2.84)&34.24(8.91)&64.24(5.88)&43.71(6.87)\\
 p = 48 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&67.57(6.37)&48.99(1.69)&63.31(1.97)&32.52(2.35)&60.29(2.35)&42.19(2.08)&67.57(6.37)&55.36(1.69)&60.74(3.17)\\
\multicolumn{1}{r}{n = 400}&55.03(5.06)&55.94(0.71)&68.51(2.36)&17.6(1.2)&66.38(3.71)&27.77(1.37)&55.03(5.06)&57.97(1.3)&56.37(2.97)\\
VAR & precision & recall & F1 & precision & recall & F1 & precision & recall & F1\\
 p = 12 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&39.54(4.59)&67.5(8.5)&56.2(5.23)&33.33(1.01)&96.67(3.12)&49.57(1.49)&39.54(4.59)&78.33(9.28)&52.09(3.83)\\
\multicolumn{1}{r}{n = 400}&38.99(3.09)&66.67(10.54)&62.9(7.07)&33.91(0.56)&100.0(0.0)&50.64(0.63)&38.99(3.09)&80.83(10.07)&52.18(2.32)\\
 p = 24 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&62.65(6.34)&30.0(2.75)&44.8(3.18)&38.27(1.1)&64.17(6.1)&47.85(2.04)&62.65(6.34)&38.96(2.43)&47.76(1.25)\\
\multicolumn{1}{r}{n = 400}&55.0(3.4)&34.79(2.24)&49.52(2.44)&35.36(0.71)&82.08(4.63)&49.4(1.31)&55.0(3.4)&50.83(2.98)&52.71(1.83)\\
 p = 48 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&85.61(3.92)&10.83(1.01)&19.47(1.61)&56.63(3.16)&31.25(4.6)&39.97(3.16)&85.61(3.92)&17.08(1.35)&28.43(1.69)\\
\multicolumn{1}{r}{n = 400}&77.93(2.88)&15.0(1.1)&25.93(1.6)&45.87(3.17)&50.47(5.07)&47.84(2.66)&77.93(2.88)&25.42(1.4)&38.28(1.36)\\
\end{tabular}}
\label{table:precision-heterogeneous}
\end{table}

==> three_metric_ho_heavy_tail_table.tex <==
\small
\begin{table}[p]
\centering
\def~{\hphantom{0}}
\tbl{Precision, Recall, F1 Score($\%$) Under Homogeneous Setting}{%
\begin{tabular}{l@{\hskip 0.4in} ccc ccc ccc}
& \multicolumn{3}{c}{Hard Thresholding}  & \multicolumn{3}{c}{Lasso} & \multicolumn{3}{c}{Adaptive Lasso}\\VMA & precision & recall & F1 & precision & recall & F1 & precision & recall & F1\\
 p = 12 & & & & & & & & & \\
\multicolumn{1}{r}{n = 100}&93.74(2.55)&55.27(2.92)&68.59(2.32)&81.34(5.27)&75.24(4.54)&73.01(3.33)&93.74(2.55)&60.6(3.76)&70.61(2.58)\\
\multicolumn{1}{r}{n = 200}&92.01(2.05)&68.01(3.71)&77.54(2.5)&75.48(4.09)&90.56(2.64)&79.0(2.63)&92.01(2.05)&76.62(3.59)&80.74(2.37)\\
 p = 24 & & & & & & & & & \\
\multicolumn{1}{r}{n = 100}&97.76(1.0)&45.67(0.88)&62.4(0.78)&88.38(3.84)&63.4(3.51)&70.54(1.62)&97.76(1.0)&50.25(1.8)&65.43(1.29)\\
\multicolumn{1}{r}{n = 200}&96.04(0.94)&52.9(1.77)&68.2(1.39)&80.27(3.14)&85.14(2.4)&79.84(2.1)&96.04(0.94)&66.25(2.23)&76.52(1.59)\\
 p = 48 & & & & & & & & & \\
\multicolumn{1}{r}{n = 100}&99.35(0.38)&43.45(0.27)&60.56(0.25)&93.98(1.77)&53.17(2.21)&66.49(1.38)&99.35(0.38)&45.43(0.91)&62.17(0.77)\\
\multicolumn{1}{r}{n = 200}&98.62(0.54)&45.67(0.79)&62.55(0.69)&88.24(1.9)&74.85(2.37)&79.04(1.36)&98.62(0.54)&55.91(1.98)&70.51(1.5)\\
 p = 96 & & & & & & & & & \\
\multicolumn{1}{r}{n = 100}&99.9(0.1)&42.95(0.07)&60.09(0.07)&98.17(0.85)&46.69(1.02)&63.01(0.74)&99.9(0.1)&43.49(0.29)&60.58(0.26)\\
\multicolumn{1}{r}{n = 200}&99.58(0.19)&43.38(0.17)&60.5(0.16)&93.47(1.11)&63.71(1.59)&74.58(1.05)&99.58(0.19)&48.68(1.02)&65.12(0.87)\\
VAR & precision & recall & F1 & precision & recall & F1 & precision & recall & F1\\
 p = 12 & & & & & & & & & \\
\multicolumn{1}{r}{n = 100}&90.01(3.06)&45.39(2.39)&57.53(1.43)&79.4(3.83)&60.27(4.04)&61.12(2.05)&90.01(3.06)&48.72(3.28)&58.25(1.67)\\
\multicolumn{1}{r}{n = 200}&89.82(0.04)&51.86(3.19)&62.49(0.97)&74.69(0.28)&73.31(0.67)&67.18(0.45)&89.82(0.04)&55.99(0.54)&64.14(0.17)\\
 p = 24 & & & & & & & & & \\
\multicolumn{1}{r}{n = 100}&94.52(1.7)&36.87(0.71)&52.65(0.52)&84.68(3.55)&48.29(2.68)&56.56(1.25)&94.52(1.7)&39.43(1.27)&53.79(0.78)\\
\multicolumn{1}{r}{n = 200}&93.62(0.65)&39.44(1.01)&55.4(0.62)&78.94(2.37)&60.72(1.69)&64.28(0.19)&93.62(0.65)&45.35(0.9)&59.14(0.7)\\
 p = 48 & & & & & & & & & \\
\multicolumn{1}{r}{n = 100}&97.79(0.98)&34.22(0.32)&50.72(0.2)&91.89(2.2)&39.39(1.13)&53.02(0.71)&97.79(0.98)&35.3(0.54)&51.41(0.4)\\
\multicolumn{1}{r}{n = 200}&97.74(0.0)&35.6(0.21)&52.26(0.19)&86.76(0.07)&49.08(0.14)&59.64(0.01)&97.74(0.0)&38.61(0.37)&54.71(0.32)\\
 p = 96 & & & & & & & & & \\
\multicolumn{1}{r}{n = 100}&98.82(0.62)&33.62(0.14)&50.22(0.09)&96.26(1.18)&35.64(0.56)&51.27(0.42)&98.82(0.62)&34.07(0.26)&50.47(0.17)\\
\multicolumn{1}{r}{n = 200}&99.43(0.12)&33.9(0.13)&50.61(0.13)&94.97(1.42)&40.39(0.84)&55.86(0.26)&99.43(0.12)&35.32(0.15)&51.99(0.11)\\
\end{tabular}}
\label{table:precision-homogeneous}
\end{table}

==> three_metric_ho_table.tex <==
\small
\begin{table}[p]
\centering
\def~{\hphantom{0}}
\tbl{Precision, Recall, F1 Score($\%$) Under Homogeneous Setting}{%
\begin{tabular}{l@{\hskip 0.4in} ccc ccc ccc}
& \multicolumn{3}{c}{Hard Thresholding}  & \multicolumn{3}{c}{Lasso} & \multicolumn{3}{c}{Adaptive Lasso}\\VMA & precision & recall & F1 & precision & recall & F1 & precision & recall & F1\\
 p = 12 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&26.78(4.17)&100.0(0.0)&54.9(11.71)&22.35(0.15)&100.0(0.0)&36.53(0.2)&26.78(4.17)&100.0(0.0)&42.09(5.01)\\
 p = 24 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&40.24(6.88)&95.62(4.24)&87.17(8.01)&15.58(1.18)&100.0(0.0)&26.94(1.76)&40.24(6.88)&99.38(1.25)&56.92(7.08)\\
 p = 48 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&67.12(7.2)&72.19(6.66)&82.06(5.0)&21.82(1.77)&100.0(0.0)&35.79(2.38)&67.12(7.2)&97.81(1.59)&79.44(5.44)\\
VAR & precision & recall & F1 & precision & recall & F1 & precision & recall & F1\\
 p = 12 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&50.28(0.34)&97.22(2.48)&69.08(2.97)&50.0(0.0)&100.0(0.0)&66.67(0.0)&50.28(0.34)&99.44(1.11)&66.79(0.47)\\
 p = 24 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&40.08(3.71)&65.83(5.93)&67.65(6.23)&27.43(0.71)&98.89(1.04)&42.94(0.83)&40.08(3.71)&81.94(4.3)&53.68(3.31)\\
 p = 48 & & & & & & & & & \\
\multicolumn{1}{r}{n = 200}&55.55(6.86)&53.06(2.83)&66.02(1.85)&20.76(2.04)&85.0(2.97)&33.3(2.43)&55.55(6.86)&65.28(2.28)&59.67(3.19)\\
\end{tabular}}
\label{table:precision-heterogeneous}
\end{table}
